MemoriesDB: A Temporal-Semantic-Relational Database for Long-Term Agent Memory / Modeling Experience as a Graph of Temporal-Semantic Surfaces

We introduce MemoriesDB, a unified data architecture designed to avoid decoherence across time, meaning, and relation in long-term computational memory. Each memory is a time-semantic-relational entity-a structure that simultaneously encodes when an event occurred, what it means, and how it connects to other events. Built initially atop PostgreSQL with pgvector extensions, MemoriesDB combines the properties of a time-series datastore, a vector database, and a graph system within a single append-only schema. Each memory is represented as a vertex uniquely labeled by its microsecond timestamp and accompanied by low- and high-dimensional normalized embeddings that capture semantic context. Directed edges between memories form labeled relations with per-edge metadata, enabling multiple contextual links between the same vertices. Together these constructs form a time-indexed stack of temporal-semantic surfaces, where edges project as directional arrows in a 1+1-dimensional similarity field, tracing the evolution of meaning through time while maintaining cross-temporal coherence. This formulation supports efficient time-bounded retrieval, hybrid semantic search, and lightweight structural reasoning in a single query path. A working prototype demonstrates scalable recall and contextual reinforcement using standard relational infrastructure, and we discuss extensions toward a columnar backend, distributed clustering, and emergent topic modeling.

==> abstracts.tex <==
arXiv version:

MemoriesDB is a unified temporal–semantic–relational database for long-term agent memory.
Each record is a time-stamped vertex with semantic embeddings and labeled edges, forming a coherent geometry of experience that integrates temporal order, meaning, and relation in a single append-only schema.
Built on PostgreSQL with pgvector extensions, the prototype supports hybrid vector–graph queries, coherence metrics, and time-bounded retrieval without specialized infrastructure.
By embedding relational structure directly into the temporal axis, MemoriesDB maintains continuity across millions of events, slowing semantic drift and restoring long-range context after topic gaps.
The system demonstrates that coherence can function as a measurable bridge between data systems and cognitive architectures, providing a substrate for agents that learn and reason over extended timelines.
This preprint presents the data model, implementation, and conceptual implications for persistent, self-referential intelligence.


public version:

MemoriesDB is a new kind of database built for minds, not rows.
Instead of storing information as disconnected facts, it treats every record as a point in a living landscape of meaning — a temporal–semantic graph where time, context, and relation are fused into one evolving geometry.
Each memory defines its own local plane of meaning; connections between them trace how understanding unfolds across time.
Running entirely on standard PostgreSQL with pgvector, MemoriesDB shows that coherence — not capacity — is the real key to long-term intelligence.
By preserving the continuity of experience, it helps AI agents remember what they’ve learned, recognize when ideas drift, and reconnect their own pasts.
It’s both a working system and a hypothesis: that intelligence grows not from how much we remember, but from how coherently those memories fit together.


twitter version:

�� Launch post (hybrid of 2 + 4)

Memory isn’t a list — it’s a shape.
MemoriesDB models experience as a layered field of meaning that folds and evolves through time.
A database that remembers coherently.
→ [arxiv.org/abs/XXXX.XXXXX]

or, a slightly more conversational variant:

What if a database could remember like a mind?
MemoriesDB treats every record as a tiny thought in time — linked by meaning, relation, and continuity.
A framework for coherent, persistent AI memory.
→ [arxiv.org/abs/XXXX.XXXXX]

�� Optional follow-up thread (2 – 3 posts)

1️⃣

Each “memory” in the system is a vertex with
– a timestamp (when)
– an embedding (what it means)
– edges (how it connects).
Together they form temporal–semantic surfaces — layers of experience where meaning flows through time.

2️⃣

Built entirely on PostgreSQL + pgvector, it merges time-series, vector, and graph logic into one schema.
No new engine, no exotic stack — just a new geometry for memory.

3️⃣

It’s both a database and a hypothesis:
that intelligence grows not from how much we remember, but from how coherently those memories fit together.
#AI #LLM #databases

